FastLLVE: Real-Time Low-Light Video Enhancement with Intensity-Aware Lookup Table

Low-Light Video Enhancement (LLVE) has received considerable attention in recent years. One of the critical requirements of LLVE is inter-frame brightness consistency, which is essential for maintaining the temporal coherence of the enhanced video. However, most existing single-image-based methods fail to address this issue, resulting in flickering effect that degrades the overall quality after enhancement. Moreover, 3D Convolution Neural Network (CNN)-based methods, which are designed for video to maintain inter-frame consistency, are computationally expensive, making them impractical for real-time applications. To address these issues, we propose an efficient pipeline named FastLLVE that leverages the Look-Up-Table (LUT) technique to maintain inter-frame brightness consistency effectively. Specifically, we design a learnable Intensity-Aware LUT (IA-LUT) module for adaptive enhancement, which addresses the low-dynamic problem in low-light scenarios. This enables FastLLVE to perform low-latency and low-complexity enhancement operations while maintaining high-quality results. Experimental results on benchmark datasets demonstrate that our method achieves the State-Of-The-Art (SOTA) performance in terms of both image quality and inter-frame brightness consistency. More importantly, our FastLLVE can process 1,080p videos at $\mathit{50+}$ Frames Per Second (FPS), which is $\mathit{2 \times}$ faster than SOTA CNN-based methods in inference time, making it a promising solution for real-time applications. The code is available at https://github.com/Wenhao-Li-777/FastLLVE.

==> tables/table1_related_works.tex <==
\begin{table}[t]
  \centering
  \caption{Different approaches for maintaining inter-frame brightness consistency.}
  \setlength{\tabcolsep}{1.5mm}{
    \begin{tabular}{cccc}
    \toprule
    Format & Method & Brightness Consistency & Real-Time \\
    \midrule
    \multirow{4}{*}{Image} & MBLLEN~\cite{lv2018mbllen} & None  & \textcolor{lightred}{\ding{55}} \\
          & DeepUPE~\cite{wang2019underexposed} & None  & \textcolor{greencolor}{\ding{51}} \\
          & DeepLPF~\cite{moran2020deeplpf} & None  & \textcolor{lightred}{\ding{55}} \\
          & Cheby~\cite{pan2022chebylighter} & None  & \textcolor{lightred}{\ding{55}} \\
    \midrule
    \multirow{6}{*}{Video} & SALVE~\cite{azizi2022salve} & None  & \textcolor{lightred}{\ding{55}} \\
          & MBLLVEN~\cite{lv2018mbllen} & 3D Convolution & \textcolor{lightred}{\ding{55}} \\
          & SMOID~\cite{jiang2019learning} & 3D Convolution & \textcolor{lightred}{\ding{55}} \\
          & SDSDNet~\cite{wang2021seeing}  & Feature Alignment & \textcolor{lightred}{\ding{55}} \\
          & SMID~\cite{chen2019seeing}  & Self-consistency & \textcolor{lightred}{\ding{55}} \\
          & StableLLVE~\cite{zhang2021learning} & Self-consistency & \textcolor{greencolor}{\ding{51}} \\
    \midrule
    Video & FastLLVE~(Ours)  &  LUT  & \textcolor{greencolor}{\ding{51}} \\
    \bottomrule
    \end{tabular}}%
  \label{tab:table1}%
  \vspace{-4mm}
\end{table}%

